Time-Continuous and Time-Discontinuous Space-Time Finite Elements for Advection-Diffusion Problems

We construct four variants of space-time finite element discretizations based on linear tensor-product and simplex-type finite elements. The resulting discretizations are continuous in space, and continuous or discontinuous in time. In a first test run, all four methods are applied to a linear scalar advection-diffusion model problem. Then, the convergence properties of the time-discontinuous space-time finite element discretizations are studied in numerical experiments. Advection velocity and diffusion coefficient are varied, such that the parabolic case of pure diffusion (heat equation), as well as, the hyperbolic case of pure advection (transport equation) are included in the study. For each model parameter set, the L2 error at the final time is computed for spatial and temporal element lengths ranging over several orders of magnitude to allow for an individual evaluation of the methods' spatial, temporal, and spacetime accuracy. In the parabolic case, particular attention is paid to the influence of time-dependent boundary conditions. Key findings include a spatial accuracy of second order and a temporal accuracy between second and third order. The temporal accuracy tends towards third order depending on how advection-dominated the test case is, on the choice of the specific discretization method, and on the time-(in)dependence and treatment of the boundary conditions. Additionally, the potential of time-continuous simplex space-time finite elements for heat flux computations is demonstrated with a piston ring pack test case.

==> Pics/cst.tex <==
\newcommand*\cols{2}
\newcommand*\rows{2}
\begin{tikzpicture}[
    scale=1,
    axis/.style={very thick, ->},
    important line/.style={thick},
    dashed line/.style={dashed, thin},
    pile/.style={thick, ->, shorten <=2pt, shorten
    >=2pt},
    every node/.style={color=black}
    ]
    %x-axis
    \draw[axis] (-0.1,0)  -- (3.5,0) node(xline)[right]{x};
    \foreach \x in {0,1,2,3}
    \draw (\x cm,0.1) -- (\x cm,-0.1) node[anchor=north] {$x_{\x}$};
    % t-axis
%    \draw[very thick] (0,-0.1) -- (0,1);
%    \draw[very thick] (0,1.3) -- (0,2.3);
    \draw[axis] (0,-0.1) -- (0,3.5) node(yline)[above]{t};
    \draw (0.1,0cm) -- (-0.1, 0cm) node[anchor=east] {$t_{0}$};
    \draw (0.1,1cm) -- (-0.1, 1cm) node[anchor=east] {$t_{1}$};
    \draw (0.1,2.0cm) -- (-0.1, 2.0cm) node[anchor=east] {$t_{2}$};
    \draw (0.1,3.0cm) -- (-0.1, 3.0cm) node[anchor=east] {$t_{3}$};
    % Lines
    \foreach \row in {0, 1, ...,\rows} {
     		\foreach \col in {0, 1, ...,\cols} {
   				 \draw[important line] (\col,\row) coordinate (A)  -- (\col+1,\row) coordinate (B);
   				 \draw[important line] (\col,\row+1) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   				 \draw[important line] (\col,\row) coordinate (A)  -- (\col,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
   				  \draw[important line] (\col+1,\row) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
   		 }
   	}
   \node (Q) at (1.5,1.5) {$Q_0$};
   \draw[thick,<-] (3,1.5cm) -- (3.5, 1.5) node[anchor=west] {$P_{0}$};
     \draw[thick,<-] (2.2,0cm) -- (3.5, 0.5) node[anchor=west] {$\Omega_l$};
        \draw[thick,<-] (2.2,3cm) -- (3.5, 2.5) node[anchor=west] {$\Omega_u$};
\end{tikzpicture}

==> Pics/fst.tex <==
\newcommand*\cols{3}
\newcommand*\rows{3}
\begin{tikzpicture}[
    scale=1,
    axis/.style={very thick, ->},
    important line/.style={thick},
    dashed line/.style={dashed, thin},
    pile/.style={thick, ->, shorten <=2pt, shorten
    >=2pt},
    every node/.style={color=black}
    ]
    %x-axis
    \draw[axis] (-0.1,0)  -- (4.5,0) node(xline)[right]{x};
    \foreach \x in {0,1,2,3,4}
    \draw (\x cm,0.1) -- (\x cm,-0.1) node[anchor=north] {$x_{\x}$};
    % t-axis
    \draw[very thick] (0,-0.1) -- (0,1);
       \draw[very thick] (0,1.3) -- (0,2.3);
    \draw[axis] (0,2.6) -- (0,4) node(yline)[above]{t};
    \draw (0.1,0cm) -- (-0.1, 0cm) node[anchor=east] {$t_{0}$};
    \draw (0.1,1cm) -- (-0.1, 1cm) node[anchor=east] {$t_{1}$};
    \draw (0.1,1.3cm) -- (-0.1, 1.3cm) node[anchor=east] {$t_{1}$};
    \draw (0.1,2.3cm) -- (-0.1, 2.3cm) node[anchor=east] {$t_{2}$};
        \draw (0.1,2.6cm) -- (-0.1, 2.6cm) node[anchor=east] {$t_{2}$};
            \draw (0.1,3.6cm) -- (-0.1, 3.6cm) node[anchor=east] {$t_{3}$};
    % Lines
    \foreach \row in {0, 1.3, ...,\rows} {
     		\foreach \col in {0, 1, ...,\cols} {
   				 \draw[important line] (\col,\row) coordinate (A)  -- (\col+1,\row) coordinate (B);
   				 \draw[important line] (\col,\row+1) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   				 \draw[important line] (\col,\row) coordinate (A)  -- (\col,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
   				  \draw[important line] (\col+1,\row) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
   		 }
   	}
	\node (Q) at (1.5,0.5) {$Q_0$};
	\node (Q) at (1.5,1.8) {$Q_1$};
	\node (Q) at (1.5,3.1) {$Q_2$};
   	\draw[thick,<-] (4,1.8cm) -- (4.5, 1.8) node[anchor=west] {$P_{1}$};
     	\draw[thick,<-] (2.2,1.3cm) -- (4.5, 1.1) node[anchor=west] {$\Omega_l$};
        \draw[thick,<-] (2.2,2.3cm) -- (4.5, 2.5) node[anchor=west] {$\Omega_u$};
\end{tikzpicture}

==> Pics/sst.tex <==
\newcommand*\cols{3}
\newcommand*\rows{3}
\begin{tikzpicture}[
    scale=1,
    axis/.style={very thick, ->},
    important line/.style={thick},
    newEdge/.style={thick, ->, >=circle},
    every node/.style={color=black}
    ]
    %x-axis
    \draw[axis] (-0.1,0)  -- (4.5,0) node(xline)[right]{x};
    \foreach \x in {0,1,2,3,4}
    \draw (\x cm,0.1) -- (\x cm,-0.1) node[anchor=north] {$x_{\x}$};
    % t-axis
    \draw[very thick] (0,-0.1) -- (0,1);
       \draw[very thick] (0,1.3) -- (0,2.3);
    \draw[axis] (0,2.6) -- (0,4) node(yline)[above]{t};
    \draw (0.1,0cm) -- (-0.1, 0cm) node[anchor=east] {$t_{0}$};
    \draw (0.1,1cm) -- (-0.1, 1cm) node[anchor=east] {$t_{1}$};
    \draw (0.1,1.3cm) -- (-0.1, 1.3cm) node[anchor=east] {$t_{1}$};
    \draw (0.1,2.3cm) -- (-0.1, 2.3cm) node[anchor=east] {$t_{2}$};
        \draw (0.1,2.6cm) -- (-0.1, 2.6cm) node[anchor=east] {$t_{2}$};
            \draw (0.1,3.6cm) -- (-0.1, 3.6cm) node[anchor=east] {$t_{3}$};
    % Lines
    \foreach \row in {0, 1.3, ...,\rows} {
     		\foreach \col in {0, 1, ...,\cols} {
   				 \draw[important line] (\col,\row) coordinate (A)  -- (\col+1,\row) coordinate (B);
   				 \draw[important line] (\col,\row+1) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
				 \draw[important line] (\col,\row) coordinate (A)  -- (\col,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
   				  \draw[important line] (\col+1,\row) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   				 \fill (A) circle (2pt);
   				 \fill (B) circle (2pt);
				  \draw[important line] (\col,\row) coordinate (A)  -- (\col+1,\row+1) coordinate (B);
   		 }			  
   	}
   	   \node (Q) at (1.325,2.0) {$Q_1$};
   \draw[thick,<-] (4,1.8cm) -- (4.5, 1.8) node[anchor=west] {$P_{1}$};
     \draw[thick,<-] (2.2,1.3cm) -- (4.5, 1.1) node[anchor=west] {$\Omega_l$};
        \draw[thick,<-] (2.2,2.3cm) -- (4.5, 2.5) node[anchor=west] {$\Omega_u$};
\end{tikzpicture}

==> Pics/ust.tex <==
\begin{tikzpicture}[
    axis/.style={very thick, ->},
    important line/.style={thick},
    dashed line/.style={dashed, thin},
    pile/.style={thick, ->, shorten <=2pt, shorten
    >=2pt},
    every node/.style={color=black}
    ]
         %x-axis
        \draw[axis] (-0.1,0)  -- (3.5,0) node(xline)[right]{x};
         \foreach \x in {0,1,2,3}
    \draw (\x cm,0.1) -- (\x cm,-0.1) node[anchor=north] {$x_{\x}$};

        % t-axis
        \draw[axis] (0,-0.1) -- (0,3.5) node(yline)[above]{t};
        \begin{axis}[axis lines=none,
        xmin = 0,
        xmax = 3,
        ymin =0,
        ymax = 3,
        x=1cm,
        y=1cm,
            	colormap={mymap}{rgb=(0,0,0); rgb=(0,0,0)}
        ]
        	  \addplot [patch, patch refines=0, mesh, thick, black, patch table={Fig/sst-triangles.txt}] table {Fig/sst-points.txt}; 
          \addplot [mark=*, only marks] table {Fig/sst-points.txt};
        \end{axis}
	\node (Q) at (1.4,1.6) {$Q_0$};
        \draw[thick,<-] (3,1.5cm) -- (3.5, 1.5) node[anchor=west] {$P_{0}$};
        \draw[thick,<-] (2.2,0cm) -- (3.5, 0.5) node[anchor=west] {$\Omega_l$};
        \draw[thick,<-] (2.2,3cm) -- (3.5, 2.5) node[anchor=west] {$\Omega_u$};
  \end{tikzpicture}

==> numExamples.tex <==
\subsection{Organization of space-time convergence study}

For each model problem, parameter set, and discretization method a space-time convergence study with 198 simulations is performed. The simulation settings are obtained as follows. We divide the time direction of the computational domain into $\nts$ space-time slabs of constant size $\Delta t = \frac{2}{\nts}$.  On each of the 15 levels of temporal refinement $\nts$ is doubled such that $\nts = 2^{m-1}, m = 4, \dots, 18$. In the same manner, the spatial domain is divided into $\nex$ elements of constant size $\Delta x = \frac{2}{\nex}$, where $\nex = 2^{l-1}, l = 4, \dots, 18$. To avoid unnecessary computational cost, we omit combinations of the finest refinement levels as shown in Figure~\ref{fig:orga}. After each simulation, the relative $L_2$ error $e_{lm}$ at final time $t_f = 2 $ for the spatial refinement level $l$ and temporal refinement level $m$ is to be determined 
\begin{align}
& e_{lm} = \frac{\| (u - u^h)(\cdot,t_f) \|}{\| u(\cdot,t_f) \|} = e^{2 \pi^2 \nu} \sqrt{\int _{\Omega_u} \left( u(x,t_t) - u^h(x,t_f) \right)^2 dx}. \nonumber
\end{align}

We approximate the $L_2$ error $e_{lm} \approx \tilde{e}_{lm}$ using element wise two point Gaussian quadrature
\begin{align}
& \tilde{e}_{lm}  =  e^{2 \pi^2 \nu}  \sqrt{ \frac{\Delta x}{2} \sum_{e=1}^{\nex}  \sum_{iq=1}^{2} \left( u(x^e_{iq},t_f) - u^h(x^e_{iq},t_f) \right)^2 }. \nonumber
 \end{align}

 Additionally, we measure the nodal errors as 
 \begin{align}
& E_{lm} \coloneqq e^{2 \pi^2 \nu} \sqrt{ \Delta x \sum_{i=1}^{\nex} \left( u(x_i,t_f) - u^h(x_i,t_f) \right)^2 }, \nonumber
 \end{align}
 with the index $i$ running over all nodes, but the last one. In problem configuration C1, node 1 and node $\nex +1$ have identical solution values enforced by the periodic boundary conditions. 
 
\newcommand{\plthgtTDT}{0.33\textheight}
\newcommand{\pltwdtTDT}{0.52\textwidth}

\begin{figure}
\centering
\begin{tikzpicture}
\begin{axis}[
	height=\plthgtTDT, width=\pltwdtTDT,
	point meta min = -9,
	zmax=0,
	zmin=-12,
	unbounded coords=jump,
	view={0}{90},
	y dir=reverse,
	colorbar right,
	xlabel=Spatial refinement level $l$,
	ylabel=Temporal refinement level $m$, 
	title=$\log (E_{lm})$,
%title style={at={(axis description cs:1.25,0.5)},anchor=north},
]
\addplot3 [surf, shader=faceted interp, mesh/rows=15, mesh/ordering=y varies, z filter/.expression= {z==-15 ? nan : z}] table [col sep=comma]  {Data/FSTQuadNu0.0L2ErrorCoords.csv};
\end{axis}
\end{tikzpicture}
\caption{Organization of space-time convergence study.}
\label{fig:orga}
\end{figure}

\subsection{Problem configuration C1}
\label{ssec:COne}

We start with the numerical error analysis for problem configuration C1. Six model parameter sets are investigated. They include the hyperbolic (pure advection) case $a = 1$, $\nu = 0.0$, next to four advection-diffusion cases with increasing viscosity $ a=1$, $\nu = 0.0001, 0.001, 0.01, 0.1$, and the parabolic (pure diffusion) case $a=0$, $\nu=0.1$. The results of the convergence studies for problem configuration C1 are visualised in Figure~\ref{fig:convADlargeE}. For the hyperbolic case, the error visualisation of the FST results (Figure~\ref{fig:convFSTNuZero}) is a continuous surface with kinks separating regions of different order of convergence. The SST results (Figure~\ref{fig:convSSTNuZero}) are similar except for the simulations with $\Delta t = \Delta x$. For these cases, the space-time finite element edges align with the characteristic curves along which the solution is transported. We observe that the finite element approximation coincides with the exact solution at the nodes (up to a round off error $\epsilon < \num{1.0e-10}$) already for the coarsest refinement level in space and time. Demkowicz and Oden describe this behaviour as `extra superconvergence`~\cite{demkowicz1986adaptive}. Comparing the parabolic cases (Figure~\ref{fig:convFSTPeZero} and Figure~\ref{fig:convSSTPeZero}), the FST discretization reaches smaller error levels. For both space-time discretizations, the advection-diffusion cases with increasing viscosity present a smooth transition from the pure advection to the pure diffusion case. 

\newcommand{\plthgtTD}{0.33\textheight}
\newcommand{\pltwdtTD}{0.52\textwidth}

\newcommand{\logPlotThreeDQuadError}[1]{
\begin{tikzpicture}
\begin{axis}
	[
	height=\plthgtTD, width=\pltwdtTD,
	point meta min = -9,
	zmax=0,
	zmin=-12,
	unbounded coords=jump,
	y dir=reverse,
	xlabel=$l$, ylabel=$m$, 
	zlabel=$\log (\tilde{e}_{lm})$,
	z label style={at={(axis description cs:0.0,0.85)},,rotate=-90,anchor=north},
	]
	\addplot3 [surf, mesh/rows=15, mesh/ordering=y varies, z filter/.expression= {z==-15 ? nan : z}] table [col sep=comma]  {Data/#1RealL2ErrorCoords.csv};
\end{axis}
\end{tikzpicture}
}

\begin{figure}
\centering
\subfloat[FST, pure advection case $a = 1$, $\nu = \num{0.0}$ \label{fig:convFSTNuZeroReal}]{\logPlotThreeDQuadError{FSTQuadNu0.0}}
\subfloat[SST, pure advection case $a = 1$, $\nu = \num{0.0}$ \label{fig:convSSTNuZeroReal}]{\logPlotThreeDQuadError{SST1DNu0.0}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.0001}$ \label{fig:convFSTNuTenThousandReal}]{\logPlotThreeDQuadError{FSTQuadNu0.0001}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.0001}$ \label{fig:convSSTNuTenThousandReal}]{\logPlotThreeDQuadError{SST1DNu0.0001}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.001}$ \label{fig:convFSTNuThousandReal}]{\logPlotThreeDQuadError{FSTQuadNu0.001}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.001}$ \label{fig:convSSTNuThousandReal}]{\logPlotThreeDQuadError{SST1DNu0.001}} \\
\end{figure} 

\begin{figure}
\centering
\ContinuedFloat 
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.01}$ \label{fig:convFSTNuHundredReal}]{\logPlotThreeDQuadError{FSTQuadNu0.01}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.01}$ \label{fig:convSSTNuHundredReal}]{\logPlotThreeDQuadError{SST1DNu0.01}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.1}$ \label{fig:convFSTNuTenReal}]{\logPlotThreeDQuadError{FSTQuadNu0.1}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.1}$ \label{fig:convSSTNuTenReal}]{\logPlotThreeDQuadError{SST1DNu0.1}} \\
\subfloat[FST, Pure diffusion case $a = 0$, $\nu = \num{0.1}$ \label{fig:convFSTPeZeroReal}]{\logPlotThreeDQuadError{FSTQuadPe0}}
\subfloat[SST, Pure diffusion case $a = 0$, $\nu = \num{0.1}$ \label{fig:convSSTPeZeroReal}]{\logPlotThreeDQuadError{SST1DPe0}} \\
\caption{Convergence visualization for problem configuration C1.}
\label{fig:convADsmallE}
\end{figure} 


\newcommand{\plthgtC}{0.4\textheight}
\newcommand{\pltwdtC}{0.47\textwidth}

\pgfplotsset{
        small e axis style/.style={
       		ymin = 2e-10, ymax = 0.5,
       		ylabel= {$\tilde{e}_{lm}$},
		grid=major,
        },
        large e axis style/.style={
       		ymin = 2e-10, ymax = 0.5,
       		ylabel= {$E_{lm}$},
		grid=major,
        }
}

\newcommand{\logPlotTwoDTimeFSTReal}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta t$},
	small e axis style,
	ymin = 5e-11, ymax = 0.5,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0RealL2ErrorTime.txt};
        \addplot[ultra thick,dashed,domain=0.001:0.25, samples=100]{(x)^(3)};
        \addplot[ultra thick,dashed,domain=0.01:0.25, samples=100]{(x)^(3)/100};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDTimeSSTReal}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       height=\plthgtC, width=\pltwdtC,
    xlabel={$\Delta t$},
	small e axis style,
	ymin = 5e-11, ymax = 0.5,
               legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\, \nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta t^2)$, $\mathcal{O}(\Delta t^3)$},
       legend to name=twoDRealTimeLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0RealL2ErrorTime.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)};
        \addplot[ultra thick,dashed,domain=0.001:0.025, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDRealTimeLegend}\\
\subfloat[FST, $\Delta x = \frac{1}{65536}$   \label{fig:convTwoDFSTTimeReal}]{\logPlotTwoDTimeFSTReal{FSTQuad}}
\subfloat[SST, $\Delta x = \frac{1}{65536}$   \label{fig:convTwoDSSTTimeReal}]{\logPlotTwoDTimeSSTReal{SST1D}}\\
\caption{Temporal convergence for C1 for six model parameter sets.}
\label{fig:twoDTimeReal}
\end{figure} 


\newcommand{\logPlotTwoDSpaceReal}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta x$},
	small e axis style,
	ymin = 1e-7, ymax = 0.5,
               legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\,\nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta x^2)$},
       legend to name=twoDRealSpaceLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0RealL2ErrorSpace.txt};
	\addplot+[ultra thick,dashed] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0RealL2ErrorSpace.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)/5};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDRealSpaceLegend}\\
\subfloat[FST, $\Delta t = \frac{1}{65536}$   \label{fig:convTwoDFSTSpaceReal}]{\logPlotTwoDSpaceReal{FSTQuad}}
\subfloat[SST, $\Delta t = \frac{1}{65536}$   \label{fig:convTwoDSSTSpaceReal}]{\logPlotTwoDSpaceReal{SST1D}}
\caption{Spatial convergence for C1 for six model parameter sets.}
\label{fig:twoDSpaceReal}
\end{figure}


\newcommand{\logPlotTwoDSpaceTimeReal}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta x = \Delta t$},
    	small e axis style,
	ymin = 1e-9, ymax = 0.5,
	legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\,\nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta t^2)$},
       legend to name=twoDSpaceTimeRealLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0RealL2ErrorSpaceTime.txt};
	\addplot[ultra thick,dotted,domain=0.0001:0.1, samples=100]{(x)^(2)/5};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDSpaceTimeRealLegend}\\
\subfloat[FST \label{fig:convTwoDFSTSpaceTimeReal}]{\logPlotTwoDSpaceTimeReal{FSTQuad}}
\subfloat[SST \label{fig:convTwoDSSTSpaceTimeReal}]{\logPlotTwoDSpaceTimeReal{SST1D}}\\
\caption{Space-time convergence for C1 for six model parameter sets.}
\label{fig:twoDSpaceTimeReal}
\end{figure} 

\newcommand{\logPlotTwoDSpaceTimeSpecialReal}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta t$},
    	small e axis style,
	legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\,\nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta t^2)$, $\mathcal{O}(\Delta t^3)$},
       legend to name=twoDSpaceTimeSpecialRealLegend,
]
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Pe0RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.1RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.01RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.001RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.0001RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.0RealL2ErrorSpaceTimeSpecial.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)};
	\addplot[ultra thick,dashed,domain=0.001:0.1, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDSpaceTimeSpecialRealLegend}\\
\subfloat[FST \label{fig:convTwoDFSTSpaceTimeSpecialReal}]{\logPlotTwoDSpaceTimeSpecialReal{FSTQuad}}
\subfloat[SST \label{fig:convTwoDSSTSpaceTimeSpecialReal}]{\logPlotTwoDSpaceTimeSpecialReal{SST1D}}\\
\caption{Space-time convergence with $\Delta x^2 = \Delta t^3$ for C1 for six model parameter sets.}
\label{fig:twoDSpaceTimeSpecialReal}
\end{figure} 


\newcommand{\logPlotThreeD}[1]{
\begin{tikzpicture}
\begin{axis}[
	height=\plthgtTD, width=\pltwdtTD,
	point meta min = -9,
	zmax=0, zmin=-12,
	unbounded coords=jump,
	y dir=reverse,
	xlabel=$l$, ylabel=$m$, 
	zlabel=$\log (E_{lm})$,
	z label style={at={(axis description cs:0.0,0.85)},,rotate=-90,anchor=north},
	]
	\addplot3 [surf, mesh/rows=15, mesh/ordering=y varies, z filter/.expression= {z==-15 ? nan : z}] table [col sep=comma]  {Data/#1L2ErrorCoords.csv};
\end{axis}
\end{tikzpicture}
}

\begin{figure}
\centering
\subfloat[FST, pure advection case $a = 1$, $\nu = \num{0.0}$ \label{fig:convFSTNuZero}]{\logPlotThreeD{FSTQuadNu0.0}}
\subfloat[SST, pure advection case $a = 1$, $\nu = \num{0.0}$ \label{fig:convSSTNuZero}]{\logPlotThreeD{SST1DNu0.0}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.0001}$ \label{fig:convFSTNuTenThousand}]{\logPlotThreeD{FSTQuadNu0.0001}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.0001}$ \label{fig:convSSTNuTenThousand}]{\logPlotThreeD{SST1DNu0.0001}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.001}$ \label{fig:convFSTNuThousand}]{\logPlotThreeD{FSTQuadNu0.001}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.001}$ \label{fig:convSSTNuThousand}]{\logPlotThreeD{SST1DNu0.001}} \\
\end{figure} 

\begin{figure}
\centering
\ContinuedFloat 
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.01}$ \label{fig:convFSTNuHundred}]{\logPlotThreeD{FSTQuadNu0.01}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.01}$ \label{fig:convSSTNuHundred}]{\logPlotThreeD{SST1DNu0.01}} \\
\subfloat[FST, advection diffusion case $a = 1$, $\nu = \num{0.1}$ \label{fig:convFSTNuTen}]{\logPlotThreeD{FSTQuadNu0.1}}
\subfloat[SST, advection diffusion case $a = 1$, $\nu = \num{0.1}$ \label{fig:convSSTNuTen}]{\logPlotThreeD{SST1DNu0.1}} \\
\subfloat[FST, Pure diffusion case $a = 0$, $\nu = \num{0.1}$ \label{fig:convFSTPeZero}]{\logPlotThreeD{FSTQuadPe0}}
\subfloat[SST, Pure diffusion case $a = 0$, $\nu = \num{0.1}$ \label{fig:convSSTPeZero}]{\logPlotThreeD{SST1DPe0}} \\
\caption{Nodal error based convergence visualisation for problem configuration C1.}
\label{fig:convADlargeE}
\end{figure} 

After this view on the convergence over the complete of range parameter values for $\Delta x$ and $\Delta t$, we now focus on spatial convergence, temporal convergence, and convergence along the space-time diagonal separately. To check for spatial convergence, we consider the finest temporal refinement level $m= 18$ and vary $l = 4 \dots 12$, which corresponds to the bottom line of the plot in Figure~\ref{fig:orga}. Analogous to investigate temporal convergence, we consider the finest spatial refinement level $l= 18$ and vary $m = 4 \dots 12$. This corresponds to the right most line of the plot in Figure~\ref{fig:orga}. On the space-time diagonal $\Delta t= \Delta x$, we consider 12 data points $m = 4 \dots 15$.

Figure~\ref{fig:twoDTime} collects the results of the temporal convergence study. FST is observed to be third order accurate with respect to the time step for the complete range of parameter sets. The SST method is third order time accurate in the hyperbolic case and of second order in the parabolic case. For advection diffusion cases we observe a convergence behaviour between second and third order. However, rather than converging at a constant rate, SST converges with third order up to $\Delta t _{turn} (\Delta x, \nu)$, where convergence transitions to second order. For larger diffusion coefficients $\nu$ the transition occurs for larger time steps, i. e., earlier in the convergence history.
 
The FST behaviour is inline with the results obtained by Shakib and Hughes in a Fourier analysis of the purely advective and purely diffusive limiting case~ \cite{shakib1991new}. Note that the specific stencil of the FST discretization is used in the Fourier analysis and the result hence does not apply to a SST discretization. In contrast, the finite element error estimate presented by Shakib and Hughes~\cite{shakib1991new} does not require a tensor product structure of the shape functions and therefore applies to SST. Despite the fact that the error estimate includes additional terms besides the $L_2$ error, the SST behaviour is in agreement with the estimate's prediction of a third order accuracy for advection dominated cases and a second order accuracy for diffusion dominated cases. 

The third order convergence of FST for the parabolic case experimentally confirms the superconvergence result of Thom\'{e}e \cite{thomee2006Galerkin} for linear elements. As pointed out by Voulis~\cite{voulis2019space} this does not hold for inhomogeneous time-dependent boundary conditions (without special treatment investigated for problem configuration C2 in Section~\ref{ssec:CTwo}). 

\newcommand{\logPlotTwoDTimeFST}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta t$},
	large e axis style,
	ymin = 5e-11, ymax = 0.5,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0L2ErrorTime.txt};
        \addplot[ultra thick,dotted,domain=0.001:0.25, samples=100]{(x)^(3)};
        \addplot[ultra thick,dashed,domain=0.01:0.25, samples=100]{(x)^(3)/100};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDTimeSST}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       height=\plthgtC, width=\pltwdtC,
    xlabel={$\Delta t$},
	large e axis style,
	ymin = 5e-11, ymax = 0.5,
               legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\, \nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta t^2)$, $\mathcal{O}(\Delta t^3)$},
       legend to name=twoDTimeLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001L2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0L2ErrorTime.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)};
        \addplot[ultra thick,dashed,domain=0.001:0.025, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDTimeLegend}\\
\subfloat[FST, $\Delta x = \frac{1}{65536}$   \label{fig:convTwoDFSTTime}]{\logPlotTwoDTimeFST{FSTQuad}}
\subfloat[SST, $\Delta x = \frac{1}{65536}$   \label{fig:convTwoDSSTTime}]{\logPlotTwoDTimeSST{SST1D}}\\
\caption{Nodal error based temporal convergence for C1 for six model parameter sets.}
\label{fig:twoDTime}
\end{figure} 

Spatial convergence results are presented in Figure~\ref{fig:twoDSpace}. The results for both space-time methods are in qualitative agreement. In the pure advection case, both methods converge with fourth order up to a $\Delta x_{turn} ( \nu)$ and then transition to second order. In the simulations with the fourth order convergence relative to each other, the element size in time direction $\Delta t$ is very small compared to $\Delta x$. In consequence, the small $\Delta t$ leads to such a small stabilization parameter $\tau$, that the influence of the SUPG term vanishes and the Galerkin method is recovered. The Galerkin method for the pure advection case is fourth order accurate with respect to $\Delta x$~ \cite{shakib1991new}. Similar to the temporal convergence study, an increasing diffusion coefficient shifts the turning point to larger $\Delta x$. In the pure diffusion case, both methods are second order accurate with respect to $\Delta x$.

\newcommand{\logPlotTwoDSpace}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       height=\plthgtC, width=\pltwdtC,
    xlabel={$\Delta x$},
	large e axis style,
	ymin = 5e-11, ymax = 0.5,
               legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\,\nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta x^2)$, $\mathcal{O}(\Delta x^4)$},
       legend to name=twoDSpaceLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0L2ErrorSpace.txt};
	\addplot+[ultra thick,dashed] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1L2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01L2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001L2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001L2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0L2ErrorSpace.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)};
        \addplot[ultra thick,dashdotted,domain=0.005:0.25, samples=100]{(x)^(4)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDSpaceLegend}\\
\subfloat[FST, $\Delta t = \frac{1}{65536}$   \label{fig:convTwoDFSTSpace}]{\logPlotTwoDSpace{FSTQuad}}
\subfloat[SST, $\Delta t = \frac{1}{65536}$   \label{fig:convTwoDSSTSpace}]{\logPlotTwoDSpace{SST1D}}
\caption{Nodal error based spatial convergence for C1 for six model parameter sets.}
\label{fig:twoDSpace}
\end{figure} 

Considering the space-time convergence along the diagonal $\Delta t = \Delta x$ (Figure~\ref{fig:twoDSpaceTime}), FST shows a third order convergence for the pure advection case. For the advection diffusion cases, we see a transition from third to second order. Again, the turning point occurs for larger $\Delta t = \Delta x$ with increasing viscosity. Figure~\ref{fig:convTwoDSSTSpaceTime} shows the `extra superconvergence` of the SST method in the pure advection case. For the five other cases, we observe a second order space-time convergence along the diagonal $\Delta t = \Delta x$.

\newcommand{\logPlotTwoDSpaceTimeFST}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta x = \Delta t$},
    	large e axis style,
	ymin = 2e-14, ymax = 0.5,
	legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=4,
       },
       legend entries={$a=0\, \nu= 0.1$, $a=1\,\nu = 0.1$, $a=1\,\nu = 0.01$, $a=1\,\nu = 0.001$, $a=1\,\nu = 0.0001$, $a=1\,\nu=0.0$, $\mathcal{O}(\Delta t^2)$, $\mathcal{O}(\Delta t^3)$},
       legend to name=twoDSpaceTimeLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0L2ErrorSpaceTime.txt};
	\addplot[ultra thick,dotted,domain=0.0001:0.025, samples=100]{(x)^(2)};
        \addplot[ultra thick,dashed,domain=0.001:0.1, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDSpaceTimeSST}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta x = \Delta t$},
    	large e axis style,
	ymin = 2e-14, ymax = 0.5,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Pe0L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.1L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.01L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.001L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0001L2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/#1Nu0.0L2ErrorSpaceTime.txt};
	\addplot[ultra thick,dotted,domain=0.0001:0.1, samples=100]{(x)^(2)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDSpaceTimeLegend}\\
\subfloat[FST \label{fig:convTwoDFSTSpaceTime}]{\logPlotTwoDSpaceTimeFST{FSTQuad}}
\subfloat[SST \label{fig:convTwoDSSTSpaceTime}]{\logPlotTwoDSpaceTimeSST{SST1D}}\\
\caption{Nodal error based space-time convergence for C1 for six model parameter sets.}
\label{fig:twoDSpaceTime}
\end{figure} 

\newcommand{\logPlotTwoDSpaceTimeSpecial}[1]{
\begin{tikzpicture}
\begin{loglogaxis}[
	height=\plthgtC, width=\pltwdtC,
    	xlabel={$\Delta t$},
    	large e axis style,
]
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Pe0L2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.1L2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.01L2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.001L2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.0001L2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/#1Nu0.0L2ErrorSpaceTimeSpecial.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.1, samples=100]{(x)^(2)};
	\addplot[ultra thick,dashed,domain=0.001:0.1, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDSpaceTimeLegend}\\
\subfloat[FST \label{fig:twoDFSTSpaceTime}]{\logPlotTwoDSpaceTimeSpecial{FSTQuad}}
\subfloat[SST \label{fig:twoDSSTSpaceTime}]{\logPlotTwoDSpaceTimeSpecial{SST1D}}\\
\caption{Nodal error based space-time convergence with $\Delta x^2 = \Delta t^3$ for problem configuration C1.}
\label{fig:twoDSpaceTimeSpecial}
\end{figure} 


\subsection{Parabolic problem configuration C2} \label{ssec:CTwo}

A major difference between FST and SST observed in Section~\ref{ssec:COne} is the temporal convergence order for the parabolic case. We want to further investigate this difference with the parabolic problem configuration C2. In this problem configuration the periodic boundary conditions of C1 are replaced by time-dependent Dirichlet boundary conditions along the space-time boundary $P_n$ (Equation~\eqref{eq:P2bc}). Figures~\ref{fig:convFSTP2} and~\ref{fig:convSSTP2} visualise the results of the space-time convergence study. For both discretization methods, the error plots result in a continuous surface. 

Focussing on the temporal convergence rates (see Figure~\ref{fig:convTwoDPTwoTime}) only of second order convergence is observed for both methods. So, we do not observe superconvergence of FST for time-dependent boundary conditions. However, with the following treatment of the boundary conditions, presented in a general setting by Voulis in~\cite{voulis2019space}, the superconvergence of the FST discretization can be recovered.

On the upper time level $\Omega_u$ of each time slab, the boundary condition is precisely evaluated.
\begin{equation}
u(-1,t_u) = u (1,t_u) = b(t_u) = - e^{-\nu \pi^2 t_u} 
\end{equation}
In contrast, on the lower time level $\Omega_l$, the boundary condition $\tilde{b}(t_l)$ is modified, such that the linear interpolation of the finite element shape functions leads to the correct analytical mean of the boundary condition
\begin{equation}
\frac{1}{2} \left[ b(t_u) + \tilde{b}(t_l) \right] \stackrel{!}{=} \frac{1}{\Delta t} \int_{t_l}^{t_u} b(t) dt.
\end{equation}
For the considered example, this means
\begin{equation}
\tilde{b}(t_l) = \left[1 + \frac{2}{\pi^{2} \nu \Delta t } \left( 1 -  e^{\pi^{2} \nu \Delta t } \right)\right] e^{- \pi^{2} \nu t_u}.
\end{equation}

For FST with $\tilde{b}(t_l)$, third order convergence is obtained (see Figure~\ref{fig:convTwoDPTwoTime}), which numerically confirms the superconvergence result of Thom\'{e}e for the FST method. For SST with $\tilde{b}(t_l)$, only quadratic convergence is observed. The lower convergence order of the SST method with treatment of the time-dependent boundary conditions hints at the fact that the superconvergence of the FST method is linked to the employed tensor product elements.  
But, also in case of the SST discretization the treatment of boundary conditions is advantageous in the sense that the error values decrease by approximately 25\%. The second-order spatial and space-time convergence of both methods is not affected by the boundary condition treatment and independent of periodic or time-dependent boundary conditions (see Figures~\ref{fig:convTwoDPTwoSpace} and~\ref{fig:convTwoDPTwoSpaceTime}). Looking at the space-time convergence for the choice $\Delta x^2 = \Delta t^3$, FST with $\tilde{b}(t_l)$ shows third order temporal accuracy (Figure~\ref{fig:convTwoDPTwoSpaceTimeSpecial}). For this parabolic case, the nodal error measure $E_{lm}$ basically shows the same results as the $L2$ error approximation $\tilde{e}_{lm}$, therefore plots of $E_{lm}$ are omitted.

\begin{figure}
\centering
\subfloat[FST \label{fig:convFSTP2}]{\logPlotThreeDQuadError{FSTQuadNu0.1P2}}
\subfloat[SST \label{fig:convSSTP2}]{\logPlotThreeDQuadError{SST1DNu0.1P2}} \\
\subfloat[FST with modified boundary condition \label{fig:convFSTP2Mod}]{\logPlotThreeDQuadError{FSTQuadNu0.1P2Mod}}
\subfloat[SST with modified boundary condition \label{fig:convSSTP2Mod}]{\logPlotThreeDQuadError{SST1DNu0.1P2Mod}} \\
\caption{Convergence visualisation for parabolic problem configuration C2.}
\label{fig:convCTwo}
\end{figure} 


\newcommand{\logPlotTwoDPTwoSpace}{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
       	xlabel={$\Delta x$},
	small e axis style
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2ModRealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2RealL2ErrorSpace.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2ModRealL2ErrorSpace.txt};
	\addplot[ultra thick,dotted,domain=0.001:0.25, samples=100]{(x)^(2)};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDPTwoTime}{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
       	xlabel={$ \Delta t$},
	small e axis style,
        legend style={
               at={(0.5,1.2)},
               anchor=north,
               cells={anchor=west},
               legend columns=6,
       },
       legend entries={FST, FST with $\tilde{b}(t_l)$, SST, SST with $\tilde{b}(t_l)$, $\mathcal{O}(\Delta x^2)$ or $\mathcal{O}(\Delta t^2)$, $\mathcal{O}(\Delta t^3)$},
       legend to name=twoDPTwoLegend,
]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2ModRealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2RealL2ErrorTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2ModRealL2ErrorTime.txt};
	 \addplot[ultra thick,dotted,domain=0.001:0.25, samples=100]{(x)^(2)/15};
         \addplot[ultra thick,dashed,domain=0.01:0.25, samples=100]{(x)^(3)/100};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDPTwoSpaceTime}{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
       	xlabel={$\Delta x = \Delta t$},
	small e axis style
	]
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/FSTQuadNu0.1P2ModRealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2RealL2ErrorSpaceTime.txt};
	\addplot+[ultra thick] table [x expr=2/(2^(\coordindex+3)), y index=0] {Data/SST1DNu0.1P2ModRealL2ErrorSpaceTime.txt};
	 \addplot[ultra thick,dotted,domain=0.0001:0.25, samples=100]{(x)^(2)};
\end{loglogaxis}
\end{tikzpicture}
}

\newcommand{\logPlotTwoDPTwoSpaceTimeSpecial}{
\begin{tikzpicture}
\begin{loglogaxis}[
       	height=\plthgtC, width=\pltwdtC,
       	xlabel={$\Delta t$},
	small e axis style,
]
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/FSTQuadNu0.1P2RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/FSTQuadNu0.1P2ModRealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/SST1DNu0.1P2RealL2ErrorSpaceTimeSpecial.txt};
	\addplot+[ultra thick] table [x expr=2^(-2*\coordindex -2), y index=0] {Data/SST1DNu0.1P2ModRealL2ErrorSpaceTimeSpecial.txt};
	 \addplot[ultra thick,dotted,domain=0.001:0.025, samples=100]{(x)^(2)/10};
	 \addplot[ultra thick,dashed,domain=0.001:0.25, samples=100]{(x)^(3)};
\end{loglogaxis}
\end{tikzpicture}
}

\begin{figure}
\centering
\ref{twoDPTwoLegend}\\
\subfloat[Spatial convergence $(\Delta t = \frac{1}{65536})$ \label{fig:convTwoDPTwoSpace}]{\logPlotTwoDPTwoSpace}
\subfloat[Temporal convergence $(\Delta x = \frac{1}{65536})$ \label{fig:convTwoDPTwoTime}]{\logPlotTwoDPTwoTime}\\
\subfloat[Space-time convergence \label{fig:convTwoDPTwoSpaceTime}]{\logPlotTwoDPTwoSpaceTime}
\subfloat[Space-time convergence $\Delta x^2 = \Delta t^3$ \label{fig:convTwoDPTwoSpaceTimeSpecial}]{\logPlotTwoDPTwoSpaceTimeSpecial}
\caption{Spatial, temporal, and space-time convergence for problem configuration C2.}
\label{fig:twoDPTwo}
\end{figure} 


==> problem.tex <==
We consider the time-dependent one-dimensional scalar linear advection-diffusion equation
 \begin{equation}
u_{,t} + a u_{,x} = \nu  u_{,xx}, \quad  x \in ]-1,1[, \quad t \in ]0,2]. \label{eq:strong}
\end{equation}
Therein, $u$ is the scalar unknown, $a$ is the advection velocity and $\nu$ denotes the diffusion coefficient. The partial derivative with respect to the time coordinate is denoted by $(.)_{,t}$, the partial derivative with respect to $x$ is denoted by $(.)_{,x}$, and the second derivative by $(.)_{,xx}$. The spatial computational domain $\Omega$ spans from $-1$ to $1$ and we consider a time interval $I = \,]0,2]$.

In problem configuration C1, 
\begin{equation}
u(x,t=0) = -\sin(\pi x)
\end{equation}
serves as initial condition. For periodic boundary conditions
\begin{equation}
u(-1,t) = u (1,t)
\end{equation}
the model problem has the analytical solution
\begin{equation}
u(x,t) = -\sin (\pi(x-at)) e^{-\nu \pi^2 t}.
\end{equation}

In problem configuration C2, we consider the parabolic case only ($a = 0$) and choose
\begin{equation}
u(x,t=0) = \cos(\pi x) \label{eq:P2ic}
\end{equation}
as initial condition. With time-dependent Dirichlet boundary conditions 
\begin{equation}
u(-1,t) = u (1,t) = - e^{-\nu \pi^2 t} \label{eq:P2bc}
\end{equation}
the model problem has the analytical solution
\begin{equation}
u(x,t) = \cos (\pi x) e^{-\nu \pi^2 t}.  \label{eq:P2sol}
\end{equation}

Both solutions are plotted in Figure~\ref{fig:config}. Problem configuration C1 is also discussed by Mojtabi and Deville~\cite{mojtabi2015one} and on a shifted computational domain by Shakib and Hughes~\cite{shakib1991new}. 

\begin{figure}
\centering
\subfloat[C1. Travelling damped sine wave with $a = 1$, $\nu= 0.1$.\label{fig:C1}]{%
\begin{tikzpicture}[
        declare function = {
            Z(\x,\y) = -sin(180*(\x-\y)) * exp(-0.987 *\y);
        }
    ]
    \begin{axis}
    [
    tick align=inside,
    domain=-1:1,
    y domain=0:2,
    samples=20, 
    minor tick num=5,
    xlabel=$x$, ylabel=$t$, zlabel=$u$,
    ]
    \addplot3 [surf] {Z(x,y)};
    \end{axis}
\end{tikzpicture}
}
\subfloat[C2. Damped cosine wave with $\nu =0.1$.\label{fig:C2}]{%
\begin{tikzpicture}[
        declare function = {
            Z(\x,\y) = cos(180*\x) * exp(-0.987 *\y);
        }
    ]
    \begin{axis}
    [
    tick align=inside,
    domain=-1:1,
    y domain=0:2,
    samples=20, % this was 200, but I changed it to 20 because of my slow PC
    minor tick num=5,
    xlabel=$x$, ylabel=$t$, zlabel=$u$,
    ]
    \addplot3 [surf] {Z(x,y)};
    \end{axis}
\end{tikzpicture}
}
\caption{Test problem configurations}
\label{fig:config}
\end{figure}

==> spacetime/Seg.tex <==
\begin{tikzpicture}
    [
	edge/.style={very thick},
	node/.style={black, draw=black, thick}
    ]

    \coordinate (a) at (3,0);
    \coordinate (b) at (5.1,0);
    
    \draw[edge] (a) -- (b);

    \fill[node] (a) circle (2.pt);
    \fill[node] (b) circle (2.pt);

\end{tikzpicture}

